Puppeteer: A Random Forest-based Manager for Hardware Prefetchers across the Memory Hierarchy

Over the years, processor throughput has steadily increased. However, the memory throughput has not increased at the same rate, which has led to the memory wall problem in turn increasing the gap between effective and theoretical peak processor performance. To cope with this, there has been an abundance of work in the area of data/instruction prefetcher designs. Broadly, prefetchers predict future data/instruction address accesses and proactively fetch data/instructions in the memory hierarchy with the goal of lowering data/instruction access latency. To this end, one or more prefetchers are deployed at each level of the memory hierarchy, but typically, each prefetcher gets designed in isolation without comprehensively accounting for other prefetchers in the system. As a result, individual prefetchers do not always complement each other, and that leads to lower average performance gains and/or many negative outliers. In this work, we propose Puppeteer, which is a hardware prefetcher manager that uses a suite of random forest regressors to determine at runtime which prefetcher should be ON at each level in the memory hierarchy, such that the prefetchers complement each other and we reduce the data/instruction access latency. Compared to a design with no prefetchers, using Puppeteer we improve IPC by 46.0% in 1 Core (1C), 25.8% in 4 Core (4C), and 11.9% in 8 Core (8C) processors on average across traces generated from SPEC2017, SPEC2006, and Cloud suites with ~10KB overhead. Moreover, we also reduce the number of negative outliers by over 89%, and the performance loss of the worst-case negative outlier from 25% to only 5% compared to the state-of-the-art.

==> definitions.tex <==
\section{Definitions}
\label{sec:defines}
To ease the understanding of the paper, in this section we define the various terms we have used throughout this paper.\break
%
\ignore{$\bullet$ \textbf{Prefetcher System Configuration (PSC) -} A PSC specifies
which prefetcher is selected at each level of the memory in the system. We denote a PSC in the form of a 4-tuple: \texttt{<prefetcher-in-L1I\$>-<prefetcher-in-L1D\$>
-<prefetcher-in-L2\$>-<prefetcher--in-LL\$>}.\ignore{For example, {\color{red}if there are two prefetchers at L1D\$, $L1D\$_{PF1}$ and $L1D\$_{PF2}$, and two prefetchers at L2\$, $L2\$_{PF1}$ and $L2\$_{PF2}$,  in a processor, then there are nine possible PSCs -- \{$L1D\$_{PF1}$=ON, $L1D\$_{PF2}$=ON, $L1D\$_{PF1,2}$=OFF\} $\times$ \{$L2\$_{PF1}$=ON, $L2\$_{PF2}$=ON, $L2\$_{PF1,2}$=OFF\}. For a system with $N_{pf}$ prefetchers at 4 memory levels, there are
$N_{psc}=(N_{pf}+1)^4$ possible PSCs.}} \break}
%
$\bullet$ \textbf{Instruction Window -} An instruction window is group of
instructions that are executed sequentially at runtime. 
At runtime, at the end of every instruction window, we run \myalgo to predict the best PSC for the succeeding instruction window.
In this work we experimented with different instruction window sizes and did not see a large change in the performance of \myalgo. 
We set the instruction window size to 100,000 instructions.\break
$\bullet$ \textbf{{PSC-Invariant Events} -}
PSC-invariant events correspond to hardware events whose values do not change with the choice of PSC.
At runtime, we calculate the average number of occurrences of a hardware event per instruction window and use these values as input features of our ML model. {\ignore{\color{black} We use hardware performance
counters (HPCs) to count the number of occurrences of various hardware-level
events in a processor.}} \break
\ignore{%
$\bullet$ \textbf{Trace -} A trace is a group of instructions that represent a
particular behavior. 
One or more traces can be used to represent the behavior
of a benchmark. 
For example, a benchmark with consistent looping behavior can be
represented by one trace corresponding to a single iteration of the loop. 
We construct one or more unique representative traces from each benchmark
\cite{perelman2003picking} to accurately represent a wide variety of different types of application behavior. }

\ignore{$\bullet$ \textbf{Baseline PSC -} This is the default PSC that we
see in real systems today. Here all prefetchers are ON and they are
controlled by the native control policies at runtime. More details are provided in
Section \ref{sec:suitap_overview}.} 
\ignore{In total, we construct 232 traces from SPEC2017, SPEC2006, and Cloud and used them to ??.}
\ignore{The number of instruction in a trace is smaller than the 100,000 instructions we have in our instruction window.}


%backup for table
\ignore{
\begin{table*}[h]
  \caption{\textbf{Comparison with prior work -} {We compare \myalgo~with prior
  work on prefetcher adapters using a variety of metrics. We use \textit{NA}
  when \color{black}the paper lacks information about the respective metric. In
  the Overhead column, for the papers that use software prefetchers, the
  overhead is not provided and so we just state ``Software''. }}
  \label{tab:prior}
\scriptsize
\renewcommand{\arraystretch}{1.0}
\centering
\begin{tabular}{P{1.2cm}|P{1.5cm}|P{2.5cm}|P{2.05cm}|P{3.8cm}|P{1.6cm}|P{2cm}|P{1.1cm}}
\hline
\textbf{Work} & \textbf{\# Prefetchers} & \textbf{IPC
Gain Over Baseline PSC} & \textbf{IPC Gain Over No Prefetching} &
\textbf{Dataset}
&
\textbf{Heuristic or Data-Driven} & \textbf{Complexity or
Adaptation}& \textbf{Overhead} \\
\hline
\hline
\cite{liao2009machine} & 4 prefetchers & Max:\missingcitation, Avg: 1.33\% & \textit{NA} & SPEC
CPU\textsuperscript \textregistered~2006 + 11 Datacenter  & Data-Driven &
Insights
from Data & Software \\
\hline
\cite{bhatia2019perceptron} & 1 prefetcher & Max:\missingcitation, Avg: 2.27\%  &
Max:\missingcitation, Avg: 15.24\% & SPEC CPU\textsuperscript \textregistered~2017 & Data-Driven & More
Complex Prefetcher Design & $\sim39$KB\\
\hline
\cite{hiebel2019machine} & 4 prefetchers & Max:\missingcitation, Avg: -1\% to 5\% & \textit{NA} &
Memory-intensive Apps from SPEC CPU\textsuperscript \textregistered~2006 and
PARSEC \cite{bienia2008parsec} & Data-Driven & Highly Dependent on Dataset&
Software\\
\hline
\cite{jimenez2012making}~ & 1 prefetcher & Max: $2.7\times$,
Avg: \textit{NA} & \textit{NA} & SPEC CPU\textsuperscript
\textregistered~2006 & Heuristic-Based & Insights
from Data & Software\\
\hline
\cite{rahman2015maximizing}~  & 4 prefetchers & Max: $1.4\times$,
Avg: \textit{NA} &\textit{NA} & PARSEC \cite{bienia2008parsec} & Data-Driven &
Insights
from Data &  Software \\
\hline
\cite{kang2013hardware}~  & 0 prefetchers & Max: 20\%, Avg: 11\% & Same & PARSEC \cite{bienia2008parsec}& Heuristic-based & Insights
from Data
 &  Software \\
\hline
\myalgo~ & 6 prefetchers & Max: 28\%, Avg: 5\% & $>50$\% & 132 Apps from 6 Data Suites &
Data-Driven & Adaptation Scheme & $\sim10$KB\\
\hline
\end{tabular}
  \vspace{-0.3in}
\end{table*}
}

==> discussion.tex <==
\section{Discussion}




==> outline.tex <==
\section*{Outline}
\begin{itemize}
    \item Introduction 
    \begin{itemize}
        \item Para stating that prefetching has been used for solving the memory latency and memory bandwidth limitations. Explain how prefetching works and that we need to find a balance between coverage, accuracy and timeliness.
        \item Discuss how a single prefetcher can provide good accuracy broadly for a set of workloads, but that prefetcher won't be suitable for a different set of workloads and that prefetcher won't be suitable for all phases of a workload. Show plots showing the performance of workloads for two different prefetchers. This can be done using Champsim. Here we need to clearly show how if we want to maximize performance, then our choice of the prefetcher varies with workload properties. Inaccurate prefetches can even increase the number of misses.
        \item Discuss the idea of having multiple prefetchers at a level in the memory hierarchy and then selecting the appropriate prefetcher at runtime. This idea of `composite prefetchers' is not new. By using composite prefetchers we can broaden the scope, what is challenging is to select the appropriate prefetcher at run-time at each level in the memory hierarchy. Most prior work has focused on prefetching for a single level of cache (either L1s or LLCs), and most of them has focused on data prefetching. We target ALL levels of the cache hierarchy as well as both instruction and data prefetching. Also, talk about the area overhead of prefetchers. We have to provide a lightweight solution.
        \item {\color{red}FURKAN: I am not sure if this fits here, what will we talk about in the related work section in this case?} Para summarizing all the prior work on the design of a `co-ordinator' or a `manager' in the prior works on composite prefetcher for a single level as well as across multiple levels. In this para we need to clearly state what are the problems/limitations of the `co-ordinator' or a `manager' in the prior works and how we are solving them.).
        \item Need to discuss what is novel about \myalgo~that differentiates it from the prior work.\\
        - Multi-core consideration with multiple prefetchers on each level.
        - Better performance vs prior work.
        - Co-optimization of both hardware overhead and increasing the IPC/ ML model accuracy.
        - Targeting adaptation of both instruction and data prefetching.
        - We get rid of negative outliers, which saves innovative ideas that could not be deployed because of their worst-case performances. It is not just the average performance that is the important metric.
        \item State the novel contributions of the paper.
    \end{itemize}

    \item Background and Related Work: \begin{itemize}
        \item Para/subsection on Why ML? The advantages to using ML compared to heuristics algorithms or not using algorithms at all. Why this problem in particular needs ML (very complicated and large solution space) and how we can leverage ML algorithms that have low overheads to get good performance compared to heuristics. How ML algorithms are more adaptable to changing environments and how ML algorithms don't have to completely reconstructed from scratch with small changes compared to heuristic algorithms which are much more hardware/environment dependent and inflexible.
        \item subsection/para on composite prefetchers and how Puppeteer is different from all the prior work that choose prefetchers at different levels in the memory hierarchy at the same time.
        \item subsection/para on ML for prefetching or ML-based prefetchers for the benefit of the reviewers.
        \item subsection on adaptation of prefetchers at runtime.
        \item subsection on using ML for adaptation of prefetchers at runtime.
        \item Table summarizing the comparisons between our work and prior adaptation algorithms.  
    \end{itemize}

    \item Suitap Design
    \begin{itemize}
        \item Suitap System Overview and Microarchitecture
        \begin{itemize}
            \item Para detailing the place Puppeteer sits w.r.t. the whole system. Draw a figure providing the system-level perspective. That Puppeteer compliments any heuristics that exist in the system. Explain that Puppeteer controls the long-term behavior and not the short-term behavior. We should also go into some explanation for prefetcher aggressiveness control methods. By stating they are essentially heuristics and that Puppeteer will compliment them as well. 
        \end{itemize}
        \item Suitap Algorithm:
        \begin{itemize}
        \item Regression vs Classification: Para explaining our method of using regression instead of classification to choose PSC. How regression is able to utilize extra information on how much quantitative benefit a certain PSC will have over other PSC. How the ML model can learn to compare the PSC and how this is a step up from just simple thresholding. An example where 0.5\% threshold can lead to major performance loss if wrongly classified. Use the fact that with classification-based approach we are missing out on the fact that different application phases need different PSCs. So we need to use a regression approach.
        \item Suite of RF Regressors vs. Single RF Regressor: Para explaining why we chose Suite of Regressors instead of a single RF Regressor. Explain how both approaches work. Discuss the advantages and disadvantages of both. Justify why we chose Suite of RF Regressors. Put in bold or italics that we chose Suite of RF Regressors.
        \item Table/Figure comparing suite of RF Regressors with single RF  Regressor,  single  RF  classifier,  suite  of  RF  classifier,single decision tree, and anything else.  Use a toy example here to justify our choice of suite of RF Regressors.
        \item Para on why NNs are not a good fit for this problem. How they have an extremely high overhead and how related papers in this field have concluded that using them directly is infeasible (Jain 2020). Note: Not sure about this one for the short paper + this might fit well into the related work section now that we have a subsection for ML there.
        \item Training Suitap: Para explaining the difficulties of training with an expo-nentially expanding execution space. Possibly a figure.
        \item Para on how we use hardware-agnostic features or micro-architecture agnostic features to solve this problem.
        \item Para on how we reduce the number of PSCs and the logic behind why we wish to reduce them.  
        \item A table to show the PSCs that we use + the final features we end up using. 
        \end{itemize}
    \item Suitap Hardware: + Figure with Microarch details + 2 paras going into the details of how the microarch design works and the power/area/performance overheads. 
    \end{itemize}
    \item Evaluation
    \begin{itemize}
        \item Methodology:
        \begin{itemize} 
        \item Para about the training methods we used for multi-core.Such as constructing the mixed-dataset and how we trained using 1C data and applied this model on a 4C system
        \item Explain champsim modifications and benchmarks that we used (SPEC and Cloud)
        \item Table with architecture and prefetchers used at each level
        \item Evaluation results
        \end{itemize}
        \begin{itemize}
            \item Single Core Results: 
            – Para comparing 1C Puppeteer model with the no-prefetcher case and other related work (L1I and L1D competitions), monolithic tree, H3 JIminez algorithm, SPP (PPF baseline) when applied to a 1C system.  Comparison will be in terms of performance improvement, accuracy, coverage, and also reduction in negative outliers. We will use box and whisker plots for comparison.
            – Para discussing how the choice of PSC changes overtime in one trace and across different traces. Show a plot of the temporal variations in the choice of PSC in a trace. Show a plot showing the distribution of the choice of PSC across different traces
            \item We will have whisker plot for the IPC and a table for the acc/coverage results. 
            \item We will have an example runtime + percentage plot to show the runtime behavior. 
            \item If space permits we will have negative outlier bar plot.
            \item Multi-core Results 
            - Para comparing 4C VTS Puppeteer model and 4C MTS Puppeteer model with (L1I and L1D competitions), monolithic tree, H3 JIminez algorithm, SPP (PPF baseline) when applied to a 4C system. Comparison will be in terms of performance improvement, accuracy, coverage, and also reduction in negative outliers. We will use box and whisker plots for comparison. 
            \item DISCUSS how we should or if we should include Puppeteer 1C Model -> 4C MTS/ 4C VTS and Vice Versa. 
            \item We will have two whisker plots 1 for 4C VTS data suite and 1 for 4C MTS data suite. The 4C MTS plot will span two columns for the four cores.
        \end{itemize}
        \item Conclusion Future work.
    \end{itemize}
\end{itemize}
